Polarizations and Hook Partitions

In this paper, we relate combinatorial conditions for polarizations of powers of the graded maximal ideal with rank conditions on submodules generated by collections of Young tableaux. We apply discrete Morse theory to the hypersimplex resolution introduced by Batzies--Welker to show that the $L$-complex of Buchsbaum and Eisenbud for powers of the graded maximal ideal is supported on a CW-complex. We then translate the "spanning tree condition" of Almousa--Fl\o ystad--Lohne characterizing polarizations of powers of the graded maximal ideal into a condition about which sets of hook tableaux span a certain Schur module. As an application, we give a complete combinatorial characterization of polarizations of so-called "restricted powers" of the graded maximal ideal.

==> figures/chains2.tex <==
% https://q.uiver.app/?q=WzAsMjAsWzUsMCwiKDMsMCwwLDApIl0sWzMsMSwiKDIsMSwwLDApIl0sWzUsMSwiKDIsMCwxLDApIl0sWzcsMSwiKDIsMCwwLDEpIl0sWzIsMiwiKDEsMiwwLDApIl0sWzMsMiwiKDEsMSwxLDApIl0sWzQsMiwiKDEsMCwyLDApIl0sWzYsMiwiKDEsMSwwLDEpIl0sWzcsMiwiKDEsMCwxLDEpIl0sWzgsMiwiKDEsMCwwLDIpIl0sWzAsMywiKDAsMywwLDApIl0sWzIsMywiKDAsMSwyLDApIl0sWzMsMywiKDAsMCwzLDApIl0sWzQsMywiKDAsMiwwLDEpIl0sWzYsMywiKDAsMSwxLDEpIl0sWzcsMywiKDAsMCwyLDEpIl0sWzgsMywiKDAsMSwwLDIpIl0sWzksMywiKDAsMCwxLDIpIl0sWzEwLDMsIigwLDAsMCwzKSJdLFsxLDMsIigwLDIsMSwwKSJdLFswLDEsIiIsMCx7ImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwyLCIiLDIseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMywiIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDcsIiIsMix7ImNvbG91ciI6WzMwLDYwLDYwXSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDgsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMyw5LCIiLDIseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzcsMTQsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSw0LCIiLDAseyJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsNSwiIiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDcsIiIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiw2LCIiLDIseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsNSwiIiwyLHsiY29sb3VyIjpbMzAsNjAsNjBdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsOCwiIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDEwLCIiLDAseyJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQsMTMsIiIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSwxNCwiIiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDExLCIiLDIseyJjb2xvdXIiOlsxMjAsNjAsNjBdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMTIsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiwxNSwiIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs3LDEzLCIiLDIseyJjb2xvdXIiOlszMCw2MCw2MF0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNywxNiwiIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDE0LCIiLDIseyJjb2xvdXIiOlsxMjAsNjAsNjBdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMTUsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwxNywiIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDE2LCIiLDEseyJjb2xvdXIiOlsxMjAsNjAsNjBdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMTcsIiIsMSx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOSwxOCwiIiwxLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDE5LCIiLDAseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsMTksIiIsMCx7ImNvbG91ciI6WzMwLDYwLDYwXSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs1LDExLCIiLDAseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	&&&&& {(3,0,0,0)} \\
	&&& {(2,1,0,0)} && {(2,0,1,0)} && {(2,0,0,1)} \\
	&& {(1,2,0,0)} & {(1,1,1,0)} & {(1,0,2,0)} && {(1,1,0,1)} & {(1,0,1,1)} & {(1,0,0,2)} \\
	{(0,3,0,0)} & {(0,2,1,0)} & {(0,1,2,0)} & {(0,0,3,0)} & {(0,2,0,1)} && {(0,1,1,1)} & {(0,0,2,1)} & {(0,1,0,2)} & {(0,0,1,2)} & {(0,0,0,3)}
	\arrow[color={rgb,255:red,92;green,92;blue,214}, no head, from=1-6, to=2-4]
	\arrow[no head, from=1-6, to=2-6]
	\arrow[no head, from=1-6, to=2-8]
	\arrow[color={rgb,255:red,214;green,153;blue,92}, no head, from=2-8, to=3-7]
	\arrow[no head, from=2-8, to=3-8]
	\arrow[no head, from=2-8, to=3-9]
	\arrow[no head, from=3-7, to=4-7]
	\arrow[color={rgb,255:red,92;green,92;blue,214}, no head, from=2-4, to=3-3]
	\arrow[no head, from=2-4, to=3-4]
	\arrow[no head, from=2-4, to=3-7]
	\arrow[no head, from=2-6, to=3-5]
	\arrow[color={rgb,255:red,214;green,153;blue,92}, no head, from=2-6, to=3-4]
	\arrow[no head, from=2-6, to=3-8]
	\arrow[color={rgb,255:red,92;green,92;blue,214}, no head, from=3-3, to=4-1]
	\arrow[no head, from=3-3, to=4-5]
	\arrow[no head, from=3-4, to=4-7]
	\arrow[color={rgb,255:red,92;green,214;blue,92}, no head, from=3-5, to=4-3]
	\arrow[no head, from=3-5, to=4-4]
	\arrow[no head, from=3-5, to=4-8]
	\arrow[color={rgb,255:red,214;green,153;blue,92}, no head, from=3-7, to=4-5]
	\arrow[no head, from=3-7, to=4-9]
	\arrow[color={rgb,255:red,92;green,214;blue,92}, no head, from=3-8, to=4-7]
	\arrow[no head, from=3-8, to=4-8]
	\arrow[no head, from=3-8, to=4-10]
	\arrow[color={rgb,255:red,92;green,214;blue,92}, no head, from=3-9, to=4-9]
	\arrow[no head, from=3-9, to=4-10]
	\arrow[no head, from=3-9, to=4-11]
	\arrow[no head, from=3-3, to=4-2]
	\arrow[color={rgb,255:red,214;green,153;blue,92}, no head, from=3-4, to=4-2]
	\arrow[no head, from=3-4, to=4-3]
\end{tikzcd}\]

==> response.tex <==
Dear Greg,

We attach the updated version of the article "Polarizations and Hook Partitions." Below we included our responses to the individual referee reports and noted some other slight changes. Please let us know if you require any further information.

Best,
Ayah Almousa and Keller VandeBogert

Report 1:
- We clarified our mdeg notation in Construction 2.3.
- We added tildes and added the word "reduced" to our description of \mathcal{C}(X;k) in Notation 2.5 and Definition 2.6 to emphasize that we are working with the reduced chain complex of X.
- We emphasized in Definition 3.3 that the complex we are defining is the L-complex.
- We corrected the mix-ups between n and d in Definitions 4.2 and 4.3. 
- The referee commented that perhaps the top nonzero module in Figure 1 should be the (d+1)st exterior power of F. However, since the rank of F is n (see Notation 3.1), we believe our figure is correct as is.
- To clarify the notation in the original Proposition 4.8, we added a Notation environment (now Notation 4.8) before it introducing the notation for min(J) and what is now first(a) (rather than what was originally called min(a)).
- We split up the original Proposition 4.8 into the statement about the acyclic matching and a corollary containing data for the A-critical cells, with a sentence in between explaining how one can deduce the new Corollary 4.10 from the proposition.
- We added the missing word "ring" in Setup 6.1.
- We corrected the indexing in Proposition 6.2.

Report 2:
- Presentation 1. We moved the original Figure 4 to now be Figure 2, appearing before Example 4.4 to clarify our notation for the locations of the vertices.
- Presentation 2. We expanded Example 4.4 to point out that the number of entries in the column of a tableau corresponds to the homological degree in which that tableau sits in the double complex. We worry that including information about the acyclic matching in this example could confuse the reader, both because we have not yet introduced the required acyclic matching yet and because this example is misleadingly simple in many ways. For this reason, we opted not to mention any discrete Morse theory in this example and instead focused on illuminating the maps appearing in the double complex of Figure 1.
- Question 1. It isn't clear a priori what the immediate connection to Sylvan resolutions is. One of the initial subtleties is that Sylvan resolutions tend to not be independent of characteristic (see for instance Example 4.3 in the linked paper). The resolutions considered here have no dependence on the characteristic of the ambient field, which makes us think that the connection might not be obvious (we are not denying such a connection exists, but also we are not well-versed enough in the material of the Eagon-Miller-Ordog paper to say for sure).  
- Copyediting 1. The notation for $L$-complexes is now consistent.
- Copyediting 2. We corrected the typo pointed out in the introduction.
- Copyediting 3. The words "Figure 3" now actually appear below Figure 3. The references to the subfigures now say 3A and 3B, matching the indexing in the actual figure.
- Copyediting 4. We added the missing word "ring" to Setup 5.2.
- Copyediting 5. We added the hyphen in "one-skeleton" in Example 5.10.

Other minor changes:
- We updated the references to reflect that the polarizations paper by Almousa, Floystad, and Lohne has been accepted to JPAA.
- We clarified in Notation 4.1 that we consider 0 to be a natural number.

==> sections/cellularity.tex <==
\section{They are cellular lol}

\begin{definition}
Let $G$ be a multigraded free $R$-module. The notation $\mdeg (G)$ denotes the set of all multidegrees of the basis elements of $G$. That is,
$$\mdeg (G) := \{ \mdeg (g) \mid g \ \textrm{is a basis element of} \ G \}.$$
\end{definition}


\begin{definition}
Let $F_\bullet$ be a multigraded complex with multigraded basis $B_i$ of each $F_i$. For any $f \in B_i$, let $(B_{i-1})_f$ denote the set of elements $b \in B_{i-1}$ maximal with respect to the property that $\mdeg (b) | \mdeg(f)$. A differential $d_i$ is \emph{induced by the multigrading} if for all multigraded basis elements $f \in B_i$, one has
$$d_i (f) = \sum_{b \in (B_{i-1})_f} \epsilon(b,f) \frac{\mdeg(f)}{\mdeg (b)} b,$$
where $\epsilon (b, f)  = \pm 1$.
\end{definition}

\begin{lemma}\label{lem:MgradedBnoes0or1}
Let $F_\bullet$ denote the multigraded minimal free resolution of a monomial ideal $I$ and let $j \geq 1$ be any integer. If all differentials $d_i$ of $F_\bullet$ with $i \leq j$ are induced by the multigrading, then 
$$\beta_{i,\alpha} (I) \leq 1 \quad \textrm{for all multidegrees} \ \alpha \ \textrm{and} \  i \leq j.$$
\end{lemma}

\begin{proof}
The proof is by induction on the homological degree $i$, where the base case $i = 0$ follows by the assumption that $F_\bullet$ is a minimal free resolution. For $i>0$, suppose that there exist two distinct basis elements $f, \ f' \in B_i$ such that $\mdeg (f) = \mdeg (f')$. By the inductive hypothesis, $(B_{i-1})_f = (B_{i-1})_{f'}$; moreover, using the fact that $d_{i-1} \circ d_i (f) = d_{i-1} \circ d_i (f') = 0$, one immediately finds that $\epsilon (g , f) = \epsilon (g,f')$ for all $g \in (B_{i-1})_f$. Thus $d_i (f- f') = 0$, contradicting the minimality of $F_\bullet$. 
\end{proof}

\begin{obs}\label{obs:CoolObs}
Let $S$ be a finite set and $i \geq 1$ any integer. Assume that $S$ may be written as a union $S = A_1 \cup \cdots \cup A_j$ with the property $|A_\ell \cap A_k| \leq 1$ for all $\ell \neq k$ and $|A_\ell | \geq i$. Then $j \geq i+1$.
\end{obs}

\begin{proof}
Assume first that $|A_\ell \cap A_k \cap A_m | = 0$ for all distinct choices $\ell, \ k , \ m$. Let $T$ denote all size $2$ subsets of $\{ A_1 , \dots , A_j \}$. There is a bijection 
$$T \to S$$
given by $\{ A_\ell , A_k \} \mapsto \textrm{the unique element of} \ A_\ell \cap A_k$. Thus $|S| = \binom{j}{2}$; moreover, by the inclusion-exclusion principle, one has 
\begingroup\allowdisplaybreaks
\begin{align*}
    |S| \geq j i - \binom{j}{2} & \implies 2 \binom{j}{2} \geq ji \\
    &\implies j \geq i+1. \\
\end{align*}
\endgroup
In the general case, one may always choose a subset of $\{ A_1 , \dots , A_j \}$ for which all triple intersections are empty, whence the result follows.
\end{proof}

\begin{theorem}
Let $I$ be a monomial ideal with linear resolution, with the property $\beta_{1, \alpha} (I) \leq 1$ for all multidegrees $\alpha$. Then the differentials of the multigraded minimal free resolution $F_\bullet$ of $R/I$ are induced by the multigrading.
\end{theorem}

\begin{proof}
The proof is by induction on the homological degree $i$ (with the base case being clear for $i = 2$). The proof follows after the establishment of a series of claims. Throughout the proof, let $F_\bullet$ denote the minimal free resolution of $R/I$.

\textbf{Claim 1:} For any $f \in B_i$ with $i \geq 2$, one has that $| \supp (d_i (f))| \geq i$.
\begin{proof}[Proof of Claim 1]
Let $f \in B_i$ be any multigraded basis element of $F_i$. By the inductive hypothesis combined with Lemma \ref{lem:MgradedBnoes0or1}, every element of $\supp (d_i (f))$ has distinct multidegree. This implies that for any two distinct $g, \ g' \in \supp (d_i (f))$, one has $| (B_{i-2})_g \cap (B_{i-2})_{g'} | \leq 1$, since if the intersection were any bigger, $g$ and $g'$ would have the same multidegree. Thus there are at most $|\supp (d_i (f))|$ sets $(B_{i-1})_g$ of cardinality at least $i-1$ (by the inductive hypothesis) with the property that $| (B_{i-2})_g \cap (B_{i-2})_{g'} | \leq 1$ for $g \neq g'$. By Observation \ref{obs:CoolObs}, $|\supp (d_i (f))| \geq i$.
\end{proof}

\textbf{Claim 2:} For any $f \in B_i$,
$$\supp (d_i (f)) = (B_{i-1})_f = \{ g \in B_{i-1} \mid \mdeg(g) | \mdeg(f) \}.$$
\begin{proof}[Proof of Claim 2]
Let $i >2$ and $f \in B_i$ be any multigraded basis element of $F_i$. Then $i \leq |\supp (d_i (f))| \leq i+1$. Assume that there exists some $g \in B_{i-1}$ with $\mdeg (g) \mid \mdeg (f)$ but $g \notin \supp (d_i (f))$. Since there are at most $i+1$ distinct degree $i$ monomials dividing $\mdeg (f)$, it follows that $|\supp (d_i (f))| \leq i$. However, for any $h \in (B_{i-2})_g$ there is a unique $g' \in B_{i-1}$ with $\mdeg (g') \mid \mdeg (f)$. Notice that $g' \notin \supp (d_i (f))$, since otherwise $d_{i-1} \circ d_i (f) \neq 0$. Thus $|\supp (d_i (f))| \leq i-1$, contradicting the claim above.
\end{proof}

Finally, it remains to show that the differential $d_i$ is induced by the multigrading. By the above, for all $f \in B_i$,
$$d_i (f) = \sum_{g \in (B_{i-1})_f} \alpha_{g,f} \frac{\mdeg (f)}{\mdeg (g)} g, \quad \textrm{for some} \ \alpha_{g,f} \in k^\times.$$
Using the fact that $d_i \circ d_{i-1} (f) = 0$ (and the assumption that $d_{i-1}$ is induced by the multigrading), it follows that for any two $g, \ g' \in (B_{i-1})_f$, $\alpha_{g,f} = \pm \alpha_{g',f}$. Thus, replacing $f$ with $\alpha_{g,f}^{-1} f$ for every $f \in B_i$, one finds that $d_i$ is induced by the multigrading. 
\end{proof}

\keller{If $\L$ is a graded lattice then $\L_i$ is all rank $i$ elements of $\L$.}

\begin{definition}
Let $\L$ denote the lcm-lattice associated to some monomial ideal $I$. Then the \emph{slimming} $\L^{\slim}$ of $\L$ is the thin subposet constructed inductively in the following manner:
\begin{enumerate}
    \item For $i=0$ or $1$, $\L^{\slim}_i = \L_i$.
    \item For $i \geq 2$, $m \in \L_i$ if and only if:
    \begin{enumerate}
        \item $(0,m) \subseteq \L^{\slim}_{\leq i-1}$, and
        \item for all $m' \in \L^{\slim}_{i-2}$ with $m' \leq m$, one has $|(m',m)| = 2$.
    \end{enumerate}
\end{enumerate}
\end{definition}

\begin{obs}
Let $\L^{\slim}$ denote the slimming of the lcm lattice of some monomial ideal $I$. Then $\L^{\slim}$ is the face poset of a cell complex.
\end{obs}

\begin{proof}
By construction, $\L^{\slim}$ is a meet-semilattice with meet given by the gcd. Any meet-semilattice is the face poset of a cell complex.
\end{proof}

\begin{theorem}
Let $I$ be a monomial ideal with linear resolution such that $\beta_{1,\alpha} (I) \leq 1$ for all multidegrees $\alpha$. Let $\L$ denote the lcm-lattice associated to $I$. Then the minimal free resolution of $I$ is supported on the cell complex associated to the slimming $\L^{\slim}$.
\end{theorem}

\begin{proof}
Observe first that if $F_\bullet$ denotes the minimal free resolution of $R/I$, then $\po (F_\bullet)$ is a subposet of $\L^{\slim}$. Moreover, in homological degrees $0$ and $1$, it is evident that $F_\bullet$ is isomorphic to the cell complex induced by $\L^{\slim}$. Now, proceed by induction on the homological degree to prove the statement.  
\end{proof}

\begin{cor}
Let $I$ be a monomial ideal with linear resolution such that $\beta_{1,\alpha} (I) \leq 1$ for all multidegrees $\alpha$. Then $I$ has minimal free resolution supported on a cell complex.
\end{cor}

\keller{Talk about the idea of "separating" multidegrees}

==> sections/isotone.tex <==
\section{Graphs of linear syzygies which induce well-defined isotone maps}\label{sec: isotone}

Both known combinatorial characterizations of polarizations of $\m^d$ in Theorem \ref{thm: polsSyzEdges} rely on the existence of the rank-preserving isotone maps $X_i$ in Construction \ref{const: pols}. However, it is not clear when a graph of linear syzygies gives rise to such a set of isotone maps.
The goal of this section is to give necessary and sufficient conditions for a graph of linear syzygies of $\m^d$ to induce isotone maps as in Construction \ref{const: pols}. These conditions, labelled (G1)-(G4), are presented in Theorem \ref{thm: isotone}.
The results in this section are a critical stepping stone in the direction of being able to generate all polarizations of $(x_1,\dots, x_n)^d$ for arbitrary $n$ and $d$.

To show that our conditions are sufficient, we give an explicit algorithm (see Construction \ref{const: isotoneMaps}) to determine a set of isotone maps from a graph of linear syzygies, and we prove in Proposition \ref{prop: algorithmWorks} that the maps output by the algorithm are indeed isotone and satisfy the condition $(*)$ in Setup \ref{set: isotone}. This algorithm extends work of Lohne in \cite{lohne2013many}, where he gives such an algorithm for determining polarizations of $(x,y,z)^d$ from potential graphs of linear syzygies. Note, however, that the three variable case is quite straightforward: any subgraph of the one-skeleton of $\cH_3^d$ containing all of the ``boundary'' edges gives rise to a set of isotone maps. As we will see in Example \ref{ex: noIsotoneMapsLcomplex}, this is not the case for $n>3$, even if the graph of linear syzygies corresponds to a set of linear syzygies in a valid free resolution of $\m^d$.

As it turns out, the main difficulty of this section is the correct formulation of the conditions (G1)-(G4) of Theorem \ref{thm: isotone}; once these conditions are written down, it is a straightforward yet tedious verification that the desired algorithm is well defined.

\begin{setup}\label{set: isotone}
Fix integers $n$ and $d$, and let $S = k[x_1,\dots, x_n]$ be a polynomial over a field $k$. Let $\Xv_i = \{x_{i1},\dots, x_{i d}\}$ be a set of variables, and let $\tilde S = k[\Xv_1,\dots, \Xv_n]$ be a polynomial ring in the union of all these variables. Denote by $\mathfrak{m} = (x_1,\dots, x_n)$ the graded maximal ideal of $S$.

Let $\Delta(n,d)$ be the dilated $(n-1)$-simplex from Definition \ref{not: dilatedSimplex}. Denote by $\Delta^\ZZ(n,d) = \Delta(n,d)\cap \ZZ^n$ the set of lattice points of the dilated simplex $d\Delta_{n-1}$, i.e., the set of tuples $\aa = (a_1,\dots, a_n)$ of non-negative integers with $\sum_i^n a_i = d$. Denote by $\sk_1(\cH^d_n)$ the one-skeleton of the hypersimplicial complex $\cH^d_n$ from Definition \ref{def: hypersimplex}. 

Let $G$ be a subgraph of $\sk_1(\cH^d_n)$. Let $\cP_i = (\Delta^\ZZ(n,d), \geq_i)$ be the poset with ground set $\Delta^\ZZ(n,d)$ and partial order $\geq_i$ from Definition \ref{def: partialOrder}, and let $\cB_d$ be the Boolean poset on $[d]$. Let $\{X_i\}_{i\in [n]}$ be a set of isotone maps
\begin{align*}
    X_i: \cP_i \ra \cB_d
\end{align*}
such that rank $k$ elements of $\cP_i$ map to rank $k$ elements of $\cB_d$ and the following property holds:
\begin{enumerate}
    \item[$(*)$]\label{cond: map} $(\cc; i,j)$ is an edge in $G$ if and only if $X_p(\cc-\epsilon_i) = X_p(\cc-\epsilon_j)$ for all $p\neq i,j$. 
    \end{enumerate}
\end{setup}

\begin{notation}\label{not: parentChild} Let $P$ be a poset and let $\aa$ and $\bb$ be elements in the ground set of $P$. The notation $\aa\gtrdot \bb$ means that $\aa$ covers $\bb$ in $P$. We will frequently say that $\aa$ is a \emph{parent} of $\bb$ and that $\bb$ is a \emph{child} of $\aa$.
\end{notation}

As the following example shows, not all subgraphs $G\subset \sk_1(\cH_n^d)$ give rise to a well-defined set of isotone maps $\{X_i\}_{i\in[n]}$ satisfying $(*)$, even if the graph corresponds to the graph of syzygies among the generators of $\m^d$ appearing in a minimal free resolution of $\m^d$.

\begin{example}\label{ex: noIsotoneMapsLcomplex}
Let $I = (x_1, x_2, x_3, x_4)^2$ in $S = k[x_1,x_2,x_3,x_4]$ where $k$ is any field. Let $\FF$ be the $L$-complex of Definition \ref{def:Lcomplexes} resolving $I$, where $\psi: F\ra S$ maps the basis element $f_i$ to the variable $x_i$.
The basis elements of $L_2^1(F)$ correspond to elements of the form $(f_{a_1}\wedge f_{a_2})\otimes (f_{b_1})$ such that $a_1<a_2$ and $a_1\leq b_1$, as described in Proposition \ref{prop:standardbasis}. Let $G_\FF$ correspond to graph of linear syzygies in the presenting step of $\FF$. Then there are no linear syzygy edges between any of the vertices corresponding to the vertices $(1,1,0,0)$, $(1,0,1,0)$ or $(1,0,0,1)$. Now, suppose there exists an isotone map $X_1: \cP_1 \ra \cB_2$ satisfying $(*)$. Then $X_1(1,1,0,0)\neq X_1(1,0,1,0)\neq X_1(1,0,0,1)$, but all must be equal to rank $1$ elements of $\cB_2$. However, $\cB_2$ has only $2$ elements of rank $1$, so this is not possible. Therefore, there is no valid set of isotone maps $X_i$ satisfying $(*)$ induced by $G_\FF$.
\end{example}

The example above gives key insights into what properties are necessary for a graph of linear syzygies to induce isotone maps. In the following theorem, we give a complete list of necessary and sufficient conditions for a graph of linear syzygies to give rise to a valid set of isotone maps satisfying $(*)$ from Setup \ref{set: isotone}. Showing necessity is a straightforward verification. Sufficiency follows from the explicit construction of these isotone maps in Construction \ref{const: isotoneMaps}.

\begin{theorem}\label{thm: isotone} Adopt notation and hypotheses of Setup \ref{set: isotone}. If $X_i$ is any map with source $\cP_i$ satisfying $(*)$, then $X_i$ is well-defined if and only if $G$ satisfies the following properties:
\begin{enumerate}[(G1)]
    \item\label{cond: complete} For any $\bb\in \cP_i$ of rank $k$, there are at most $k$ connected components of $\LS_i(\bb-\epsilon_i)$ (see Notation \ref{not: LS}), and each is a complete graph.
    \item\label{cond: twoParents} Any element of $\cP_i$ has at most two parents which are not adjacent in $G$ who share a parent.
    \item\label{cond: 1parent1child} Suppose that $\aa$ and $\bb$ both cover elements $\ff$ and $\bfg$ such that $\ff$ and $\bfg$ are in two distinct connected components of $\LS_i(\cc-\epsilon_i)$ for some $\cc$. Then $\aa$ and $\bb$ must be adjacent. Similarly, if $\aa$ and $\bb$ are covered by elements $\ff$ and $\bfg$ such that $\ff$ and $\bfg$ are in two different connected components of $\LS_i(\cc-\epsilon_i)$ for some $\cc$, then $\aa$ and $\bb$ are adjacent.
    \item\label{cond: transitive} Suppose $\ff$ and $\bfg$ are adjacent in $G$. Let $\ff$ be a parent of elements $\aa$ and $\dd$ in $\cP_i$ and let $\bfg$ be a parent of elements $\bb$ and $\dd$. If $\dd$ and $\aa$ are adjacent in $G$ and $\aa$ and $\bb$ are adjacent in $G$, then $\dd$ must also be adjacent to $\bb$ in $G$ (see Figure \ref{fig: G4}).
\end{enumerate}
\end{theorem}

\input figures/G4.tex

\begin{proof}
The existence of $X_i$ given conditions (G1)-(G4) follows from Construction \ref{const: isotoneMaps}. Now suppose that $G$ does not satisfy any of conditions (G1)-(G4) in Theorem \ref{thm: isotone}.
\begin{enumerate}[(G1)]
    \item Let $\aa$ be an element of rank $k$ in $(\Delta^\ZZ(n,d),\geq_i)$. It has at most $n-1$ children. In $\cB_d$, any element of rank $k$ has $\binom{k}{k-1} = k$ children. If $\LS_i(\aa-\epsilon_i)$ has more than $k$ components, then each component must map to a distinct descendant of a rank $k$ element of $\cB_d$, which is not possible. Moreover, if any of these connected components are not a complete graph, then there are two vertices $\aa$ and $\bb$ which are not adjacent but map to the same element of $\cB_d$, contradicting the assumption that $X_i$ satisfies $(*)$.
    \item Suppose $\aa$ has three non-adjacent parents $\bb_1, \bb_1, \bb_3\in \cP_i$ of rank $k$. If $\bb_1, \bb_2,$ and $\bb_3$ all share a parent, then $\abs{X_i(\bb_1)\cap X_i(\bb_2) \cap X_i(\bb_3)} = k-2$. But $X_i(\aa) = X_i(\bb_1)\cap X_i(\bb_2) \cap X_i(\bb_3)$, so it cannot map to a rank $k$ element of $\cB_d$, a contradiction.
    \item Suppose $\aa$ and $\bb$ are rank $k>0$ elements of $(\Delta^\ZZ(n,d), \geq_i)$ and $\aa$ is not adjacent to $\bb$. Then $X_i(\aa)\cup X_i(\bb)$ is a rank $k+1$ element of $\cB_d$. In particular, there is exactly one possible image under the map $X_i$ for a parent of both $\aa$ and $\bb$. Similarly, $X_i(\aa)\cap X_i(\bb)$ is a rank $k-1$ element of $\cB_d$, which must correspond to the image of any child of $\aa$ and $\bb$ under $X_i$.
    \item  Suppose $\aa$ is adjacent to $\dd$ and $\bb$. If $X_i$ satisfies condition $(*)$, then $X_i(\aa) = X_i(\bb)$ if and only if $\aa$ and $\bb$ are adjacent in $G$.
    \end{enumerate}
\end{proof}

The following lemma tells us that the ``boundary edges'' of the dilated simplex must be contained in the graph of linear syzygies in order for it to give rise to a set of isotone maps.

\begin{lemma}\label{lem: boundary} Adopt notation and hypotheses of Setup \ref{set: isotone}, and assume $G$ satisfies conditions (G1)-(G4) in Theorem \ref{thm: isotone}. Then for all $0\leq k\leq d$, the edge $(k\epsilon_i + (d-k+1)\epsilon_j\, ; i,j)$ is in $G$.
\end{lemma}

\begin{proof}
This follows from property \ref{cond: complete} in Theorem \ref{thm: isotone}.
\end{proof}

It turns out that this property is both necessary and sufficient in the case where $n=3$ for isotone maps $X_i$ satisfying $(*)$ to exist.

\begin{obs}
It is straightforward to verify that if $n=3$, any graph of linear syzygies such that the only edges removed from $\sk_1(\cH_3^d)$ are those contained in maximal down-triangles satisfies conditions (G1)-(G4) above.
\end{obs}

We now partition $(\Delta^\ZZ(n,d), \geq_i)$ into a set of chains we call $\cC^\pp$ such that for all $\aa\in \cC^\pp$, one has that $a_k = p_k$ for all $k\neq i,j$ (where $j=2$ if $i=1$, and $j=1$ for all other $i$). In particular, every element of $\Delta^\ZZ(n,d)$ is contained in a unique $\cC^\pp$. 
All of these chains can be extended in a natural way to maximal chains which we call $\overline{\cC^p}$. We also define a total ordering $\prec$ on the chains $\cC^\pp$ and $\overline{\cC}^\pp$ which will later be used to construct the desired $X_i$ maps in Construction \ref{const: isotoneMaps}.

\begin{notation}
If $\cC$ is any chain in $(\Delta^\ZZ(n,d), \geq_i)$, denote by $\cC_k$ the unique rank $k$ element of $\cC$, if it exists. For simplicity, if $i=1$, set $j=2$; for $i\neq 1$, set $j=1$. Denote by $\zero = (0,\dots, 0)\in \NN^n$. For any $\pp\in \NN^n$, let $\abs{\pp} = p_1+p_2+\dots+p_n$.
\end{notation}

\begin{definition}\label{def: chains}
% Define $\cC^\zero$ to be the $d$-chain 
% $$
% (\; d\epsilon_j \quad \lessdot_i \quad (d-1)\epsilon_j + \epsilon_i \quad \lessdot_i \quad \dots \quad \lessdot_i \quad \epsilon_j + (d-1)\epsilon_i \quad \lessdot_i \quad d\epsilon_i\;)
% $$
% in $(\Delta^\ZZ(n,d),\geq_i)$. In particular, this chain contains all elements $\aa\in (\Delta^\ZZ(n,d),\geq_i)$ such that $a_k = 0$ for all $k\neq i,j$.
Let $\pp\in \NN^n$ with $i,j\notin \Supp(\pp)$ and $\abs{\pp} = r \leq d$. Define $\cC^{\pp}$ to be the $(d-r)$-chain such that $\cC^{\pp}_{k-r} = \cC^\zero_k - r\epsilon_i + \pp$. In particular, every $\aa\in \cC^\pp$ satisfies that $a_k = p_k$ for all $k\neq i,j$. 

For any $\cC^{\pp}$ with $\abs{\pp} = r$, where $1\leq r\leq d$, set $m \coloneqq \min\{\ell\mid \ell\in\Supp(\pp)\}$. Let $\bar{\cC}^{\pp}$ denote the maximal chain from extending $\cC^{\pp}$ such that $\bar{\cC}^{\pp}_k = \bar{\cC}^{\pp-\epsilon_m}$ for all $k>d-r$.

% For any $\pp,\qq\in \Delta^\ZZ(n,d-r)$ with $i,j\notin \Supp(\pp+\qq)$, define the partial order $\prec$ where $\pp\prec\qq$ if $p_\ell < q_\ell$ for the first $\ell$ where they differ. 
If $\pp,\qq \in \NN^n$ with $i,j\notin \Supp(\pp+\qq)$ and $\abs{\pp}, \abs{\qq} \leq d$, define the total order $\prec$ on the chains $\cC^\pp$ where $\cC^{\pp}\prec \cC^{\qq}$ if $\abs{\pp}<\abs{\qq}$ or $\abs{\pp}=\abs{\qq}$ and $p_\ell < q_\ell$ for the first $\ell$ where they differ. Similarly, define $\overline{\cC}^\pp \prec \overline{\cC}^\qq$ if $\cC^\pp \prec \cC^\qq$. 
% Observe that every element $\aa$ in the chain $\cC^\pp$ have the same final $n-2$ entries, which coincide exactly with $\pp$. 
\end{definition}

\input{figures/chains}

\begin{example}\label{ex: chains} Figures \ref{fig: chains} and \ref{fig: 4chains} give labeled chains for $\Delta^\ZZ(3,3)$ and $\Delta^\ZZ(4,3)$, respectively. Observe that if $\aa = d\epsilon_k$ for some $k\neq i,j$, then $\aa$ is contained in the unique one-element chain $\cC^{d\epsilon_k}$. In Figure \ref{fig: 4chains}, the chains are ordered as follows:
$$
\cC^\zero \prec \cC^{\epsilon_3} \prec \cC^{\epsilon_4} \prec \cC^{2\epsilon_3} \prec \cC^{\epsilon_3+\epsilon_4} \prec \cC^{2\epsilon_4} \prec \cC^{3\epsilon_3} \prec \cC^{3\epsilon_4}.
$$
\end{example}

\begin{notation}\label{not: booleanChains} Elements of the symmetric group $\mathfrak{S}_d$ correspond bijectively to chains of $\cB_d$ via
\begin{equation}\label{eq: wordToChain}
\sigma \mapsto (\emptyset\subset \{\sigma_1\}\subset \{\sigma_1,\sigma_2\}\subset \dots \subset \{\sigma_1,\dots, \sigma_d\}).
\end{equation}
One may also view $\sigma$ as a word in $[d]$. Set $\sigma\vert_\ell$ to be the subword $(\sigma_1,\dots, \sigma_\ell)$ of $\sigma$. Then $\sigma\vert_\ell$ corresponds to a chain of length $\ell$ in $\cB_d$ via
$$
\sigma\vert_\ell \mapsto (\emptyset\subset \{\sigma_1\}\subset \{\sigma_1,\sigma_2\}\subset \dots \subset \{\sigma_1,\dots, \sigma_\ell\}).
$$
For any two words $\tau,\sigma$, say that $\tau\subseteq\sigma$ if for all $i$, there exists some $j$ such that $\tau_i = \sigma_j$.

When referring to the image of $\aa\in (\Delta^\ZZ(n,d),\geq_i)$ under a map $X_i$, say that $\aa$ is \emph{labeled by} the element $X_i(\aa)\in \cB_d$. Given a chain $\cC$ of $(\Delta^\ZZ(n,d),\geq_i)$, say that $\cC$ is \emph{labeled by} $\sigma\in \mathfrak{S}_d$ if $X_i(\cC_k) = \{\sigma_1, \sigma_2,\dots, \sigma_k\}$.
\end{notation}

The following construction generalizes work of Lohne in \cite{lohne2013many}. The idea is to label the maximal chains $\overline{\cC^\pp}$ in the order $\prec$ presented in Definition \ref{def: chains}, starting at the bottom of each chain. Every time an element of $\aa \in \cC^\pp$ is not adjacent to the previously labeled element of the same rank in a specified earlier chain, one must apply a transposition to the word that labeled that chain.

\begin{construction}\label{const: isotoneMaps} Adopt notation and hypotheses of Setup \ref{set: isotone}, and assume $G$ satisfies conditions (G1)-(G4) of Theorem \ref{thm: isotone}. Begin by labeling the chain $\cC^\zero$ by the word $\sigma^\zero = (12\dots d)\in \mathfrak{S}_d$. 
% Now, label all $\overline{\cC}^{\pp}$ such that $\abs{\pp} = 1$ as follows.
% Observe that each $\overline{\cC}^{\pp}_k$ shares the parent $\cC^{\zero}_{k+1}$ with $\cC^\zero_k$. 
% If $\overline{\cC}^{\pp}_k$ is adjacent (or equal) to $\cC^\zero_k$ for all $k$, then label the chain $\overline{\cC}^{\pp}$ by $\sigma^\pp = \sigma^\zero$. Otherwise, starting with $k=0$, for every $k$ such that $\overline{\cC}^{\pp}_k$ is not adjacent (or equal) to $\cC^\zero_k$, apply the transposition $(k,k+1)$ to $\sigma^\zero$ to obtain the new word $\sigma^\pp$.
% $$
% \sigma^{\pp} = \left(\prod_{\cC^\zero_k, \overline{\cC}^{\pp}_k \text{not adjacent}} (k,k+1) \right)\cdot \sigma^\zero.
% $$
% Label the chain $\cC^\pp$ by $\sigma^\pp$.
% Continue to
Label all chains $\cC^\pp$ in increasing order with respect to $\prec$ in Definition \ref{def: chains} as follows. For any $\cC^{\pp}$ with $\abs{\pp} = r$, where $1\leq r\leq d$, set $m \coloneqq \min\{\ell\mid \ell\in\Supp(\pp)\}$. Starting at $k=0$, apply the transposition $(k,k+1)$ to $\sigma^{\pp-\epsilon_m}$ for every $k$ such that $\cC^{\pp}_k$ is not adjacent to $\cC^{\pp-\epsilon_m}_k$. Let $\sigma^\pp$ be the resulting word in $\mathfrak{S}_d$ after applying all required transpositions, and label the chain $\overline{\cC}^{\pp}$ by the word $\sigma^{\pp}$.
% $$
% \sigma^{\pp} = \left(\prod_{\overline{\cC}^{\pp-\epsilon_m}_k, \overline{\cC}^{\pp}_k \text{not adjacent}} (k,k+1)\right) \cdot \sigma^{\pp-\epsilon_m}.
% $$
% Label each chain $\overline{\cC}^{\pp}$ by the word $\sigma^{\pp}$.
% This process is summarized in Algorithm \ref{alg: isotone}.
\end{construction}

% \begin{algorithm}[H]\label{alg: isotone}
% \SetAlgoLined
% \KwResult{An isotone map $X_i: (\Delta^\ZZ(n,d), \geq_1)\ra \cB_d$ satisfying $(*)$ in Setup \ref{set: isotone}.}
% $G_\FF$ a graph of linear syzygies for $(x_1,\dots, x_n)^d$ satisfying $(G1)-(G4)$ in Theorem \ref{thm: generalizedPols}\;
% $\sigma^\zero = (12\dots d)$\;
% \For
% \caption{Algorithm to produce an isotone map $X_1$ from a graph of linear syzygies satisfying the Conditions (G1)-(G4) of Theorem \ref{thm: isotone}.}
% \end{algorithm}
% \begin{algorithm}[H]\label{alg: isotone}
% \SetAlgoLined
% \KwResult{An isotone map $X_i: (\Delta^\ZZ(n,d), \geq_1)\ra \cB_d$ satisfying $(*)$ in Setup \ref{set: isotone}.}
% $G_\FF$ a graph of linear syzygies for $(x_1,\dots, x_n)^d$ satisfying $(G1)-(G4)$ in Theorem \ref{thm: generalizedPols}\;
% $\sigma^\zero = (12\dots d)$\;
% \For{$\pp\in \NN^n$}{
%     \For{$\pp\in\Delta^\ZZ(n,d-r)$ such that $\{i,j\}\notin\Supp(\pp)$}{
%         $m \coloneqq \min\{\ell\mid \ell\in\Supp(\pp)\}$\;
%         $\sigma^{\pp} \coloneqq \sigma^{\pp-\epsilon_m}$\;
%         \While{$k<d-r$}{
%             \If{$\overline{\cC}^{\pp}_k$ is not adjacent to $\overline{\cC}^{\pp-\epsilon_m}_k$}
%                 {$\sigma^{\pp} = (k,k+1)\sigma^{\pp}$\;}
%         }
%     \Return $X_i(\bar{\cC}^{\pp}) = \sigma^{\pp}$\;
% }
% }
% \caption{Algorithm to produce an isotone map $X_1$ from a graph of linear syzygies satisfying the Conditions (G1)-(G4) of Theorem \ref{thm: isotone}.}
% \end{algorithm}

\input{figures/3varAlgEx}
\begin{example}\label{ex: isotoneChains} We apply the algorithm in Construction \ref{const: isotoneMaps} to the graph of linear syzygies in Figure \ref{fig: 3varAlgEx} for $(x,y,z)^3$, which is a subgraph of the one-skeleton of $\cH^d_n$ in Figure \ref{fig: dilatedSimplex}. The chains in $(\Delta^\ZZ(3,3),\geq_1)$ are labeled in Figure \ref{fig: chains}. First, set $\sigma^\zero = (123)$ by construction. To find $\sigma^{\epsilon_3}$, observe that the rank $1$ and rank $2$ elements of $\cC^{\epsilon_3}$ are not adjacent to the rank $1$ and $2$ elements of $\cC^\zero$. So $\sigma^{\epsilon_3} = (23)(12)\sigma^\zero = (23)(12)(123) = (23)(213) = (231)$. Similarly, to compute $\sigma^{2\epsilon_3}$, observe that the rank $1$ element of $\cC^{2\epsilon_3}$ is not adjacent to the rank $1$ element of $\cC^{\epsilon_3}$, so $\sigma^{2\epsilon_3} = (12)(231) = (321)$.
\end{example}

\begin{remark} Let $\aa\in \Delta^\ZZ(n,d)$. Then $\aa$ appears in the unique chain $\cC^{\pp}$ where $\abs{\pp} = d-a_i-a_j$ and $\pp = \displaystyle \sum_{\ell \neq i,j} a_\ell \epsilon_\ell$. Moreover, observe that $\sigma^\pp_k = \sigma^{\pp-\epsilon_m}_k$ for all $k > d-\abs{\pp}$ by construction. In particular, every $\aa\in (\Delta^\ZZ(n,d),\geq_i)$ is given a unique labeling by Construction \ref{const: isotoneMaps}, so it is well-defined.
\end{remark}

We conclude this section by checking that the rank-preserving maps $X_i$ produced by Construction \ref{const: isotoneMaps} are indeed isotone maps and satisfy $(*)$ from Setup \ref{set: isotone} if $G$ satisfies condition (G1)-(G4) in Theorem \ref{thm: isotone}. The proof follows from a double induction on the chains $\cC^\pp$ (following the order $\prec$ from Definition \ref{def: chains}) as well as the rank $k$ on $\cC^\pp$.

\begin{prop}\label{prop: algorithmWorks} Adopt notation and hypotheses of Setup \ref{set: isotone}, and assume $G$ satisfies conditions (G1)-(G4) in Theorem \ref{thm: isotone}. Let $\{X_i\}_{i\in [n]}$ be a set of maps from $\Delta^\ZZ(n,d)$ to $\cB_d$ as in Construction \ref{const: isotoneMaps}. Then
\begin{enumerate}[(i)]
    \item every map $X_i: (\Delta^\ZZ(n,d), \geq_i) \ra \cB_d$ is isotone, and
    \item $(\cc; s,t)$ is an edge in $G$ if and only if $X_i(\cc-\epsilon_s) = X_i(\cc-\epsilon_t)$ for all $i\neq s,t$.
\end{enumerate}
\end{prop}

\begin{proof}
Proceed by induction on the chains $\cC^{r,\pp}$ and the rank $k$ of the poset. For ease of notation, assume that $i=1$.

\noindent\textbf{Base case.} Construction \ref{const: isotoneMaps} labels the chain $\cC^\zero$ in an isotone manner by construction. The next chain labeled by the algorithm is $\overline{\cC}^{\epsilon_3}$. By construction, every element $\aa\in \cC^{\epsilon_3}$ will satisfy $X_1(\aa) = X_1(\aa - \epsilon_3 + \epsilon_2)$ if and only if $\aa$ is adjacent to $\aa-\epsilon_3+\epsilon_2$, and $X_1(\aa) \subset X_1(\aa+\epsilon_1-\epsilon_3)$ by construction, as well.

For any other chain $\cC^{\pp}$, Construction \ref{const: isotoneMaps} will always label the bottom element $\cC^{\pp}_0$ with the empty set, so its image under $X_1$ will always be less than the image of any element above it in $\cP_1$ under $X_1$. Moreover, by Lemma $\ref{lem: boundary}$, every edge on the boundary of $\sk_1(\cH^d_n)$ is in $G$, so all elements of rank $0$ also satisfy condition (ii).

\noindent\textbf{Induction hypothesis.} Assume that all chains preceding $\overline{\cC}^{\pp}$ have been labeled by Construction \ref{const: isotoneMaps}, and that all elements in these preceding chains satisfy (i) and (ii) with respect to other elements in chains preceding $\overline{\cC}^{\pp}$. Moreover, for any $\aa' = \overline{\cC}^{\pp}_\ell$ with $\ell< k$, assume $\aa'$ satisfies properties (i) and (ii) with respect to other elements in $\cP_1$ in earlier chains.

\input{figures/InductionProofIsotinicity}

\noindent\textbf{Induction Step.} Let $\aa = \overline{\cC}^{\pp}_k = \cc-\epsilon_s$ for $\cc\in\Delta^\ZZ(n,d+1)$ and some $s\in[n]$. Set $m\coloneqq \min\{\ell \mid \ell\in\Supp(\aa) \text{ and } \ell\neq 1,2\}$.

\vspace{1em}
\noindent\underline{\emph{Proof of (i).}} It suffices to check (i) in the case when $\dd = \aa + \epsilon_1 - \epsilon_t$ is a cover of $\aa$ in $\cP_1$, where $t\in\Supp(\aa)$. This situation is depicted in Figure \ref{fig: isotoneInduction}. If $t = 2$ or $m$, then $X_1(\aa) < X_1(\aa + \epsilon_1 - \epsilon_t)$ by construction, so assume $t\neq 2,m$. Observe that $\aa + \epsilon_1 - \epsilon_m$ also covers $\aa$ and shares a parent with $\aa + \epsilon_1 - \epsilon_t$, namely, $\aa+2\epsilon_1 - \epsilon_m - \epsilon_t$. If $\aa + \epsilon_1 - \epsilon_t$ is adjacent to $\aa+\epsilon_1 - \epsilon_m$, then by the induction hypothesis $X_1(\aa + \epsilon_1 - \epsilon_t) = X_1(\aa + \epsilon_1 - \epsilon_m)$ and so $X_i(\aa) < X_i(\aa + \epsilon_1 - \epsilon_t)$.

Assume $\aa + \epsilon_1 - \epsilon_t$ is not adjacent to $\aa+\epsilon_1 - \epsilon_m$. The element $\aa + \epsilon_1 - \epsilon_t$ also covers $\aa - \epsilon_t + \epsilon_2$, and the element $\aa + \epsilon_1 - \epsilon_m$ also covers $\aa + \epsilon_2 - \epsilon_m$. Moreover, $\aa + \epsilon_2 - \epsilon_m$ and $\aa + \epsilon_2 - \epsilon_t$ are both covered by $\hh = \aa - \epsilon_t + \epsilon_j - \epsilon_m + \epsilon_1$. All of the elements in the set $S = \{\aa, \aa + \epsilon_2 - \epsilon_m, \aa + \epsilon_2 - \epsilon_t\}$ cover the element $\aa - \epsilon_1 + \epsilon_2$; so by Condition \ref{cond: twoParents} in Theorem \ref{thm: isotone}, at least two elements of $S$ must be adjacent. 
Because of the assumption that $\aa + \epsilon_1 - \epsilon_t$ is not adjacent to $\aa+\epsilon_1 - \epsilon_m$, one has by Condition \ref{cond: 1parent1child} that if any pair of element of $S$ are adjacent in $G$, then all three must be pairwise adjacent.
By construction, $X_1(\aa) = X_1(\aa+\epsilon_2 - \epsilon_m)$ if and only if they are adjacent in $G$; and by the induction hypotheses, $X_1(\aa+\epsilon_2 - \epsilon_m)= X_1(\aa+\epsilon_2 - \epsilon_t)$ if and only if they are adjacent in $G$. Because all three are adjacent, one has $X_1(\aa) = X_1(\aa + \epsilon_2 - \epsilon_t) < X_1(\aa + \epsilon_1 - \epsilon_t)$, giving the desired result.

\noindent\underline{\emph{Proof of (ii).}} It suffices to check (ii) in the case when $\bb = \cc-\epsilon_t$ is in a chain preceding $\cC^{\pp}$. There are two possible cases to check: when $t = m$ (see Figure \ref{fig: iicase1}), and when $t\neq m$ (see Figure \ref{fig: iicase2}). 
\input{figures/inductionCase1}

\begin{itemize}
\item $\mathbf{t = m, (\implies):}$ Assume $\aa$ is adjacent to $\bb$. Let $\dd = \aa - \epsilon_m + \epsilon_2$. All three elements $\aa, \bb$, and $\dd$ are children of the element $\aa + \epsilon_1 -\epsilon_m$. 
If $\dd$ is adjacent to either $\aa$ or $\bb$, then all three must be adjacent by \ref{cond: complete}.
By construction, $X_1(\aa) = X_1(\dd)$, and by induction, $X_1(\dd) = X_1(\bb)$; so $X_1(\aa) = X_1(\bb)$, as desired.

Now suppose that $\dd$ is adjacent to neither $\aa$ nor $\bb$. The element $\aa - \epsilon_1 + \epsilon_2$ is covered by both $\aa$ and $\dd$, and the element $\bb-\epsilon_1+\epsilon_2$ is covered by both $\bb$ and $\dd$. Therefore, $\aa-\epsilon_1 + \epsilon_2$ must be adjacent to $\bb-\epsilon_1 + \epsilon_2$ by Condition \ref{cond: 1parent1child} in Theorem \ref{thm: isotone}. By the induction hypothesis, $X_1(\aa-\epsilon_1+\epsilon_2) = X_1(\bb-\epsilon_1 + \epsilon_2)$. In addition, $X_1(\aa), X_1(\bb),$ and $X_1(\dd)$ must all contain $X_1(\aa-\epsilon_1 + \epsilon_2)$ and be contained in $X_1(\aa + \epsilon_1 - \epsilon_m)$ by induction (for $\bb$ and $\dd$) and by construction (for $\aa$), so there are only two possible options for labels for $\aa,\bb,$ and $\dd$. Since $X_1(\dd) \neq X_1(\aa)$ by construction and $X_1(\dd)\neq X_1(\bb)$ by induction, one has that $X_1(\aa) = X_1(\bb)$, as required.

\item $\mathbf{t = m, (\impliedby):}$ Suppose $\aa$ is not adjacent to $\bb$. By Conditon \ref{cond: complete}, at most one of the pair $(\aa,\bb)$ may be adjacent to $\dd$. If one is connected to $\dd$ and the other is not, then $X_1(\aa)\neq X_1(\bb)$ by construction. Now suppose that neither $\aa$ nor $\bb$ is connected to $\dd$. Then $\bb - \epsilon_1 + \epsilon_2$ is not adjacent to $\aa - \epsilon_1 + \epsilon_2$, since otherwise $G$ would violate Condition (\ref{cond: twoParents}) in Theorem \ref{thm: isotone}. By construction, $X_1(\aa)\cap X_1(\dd) = X_1(\aa - \epsilon_1 + \epsilon_2)$, and by induction $X_1(\bb) \cap X_1(\dd) = X_1(\bb - \epsilon_1 + \epsilon_2)$. Since $X_1(\aa - \epsilon_1 + \epsilon_2) \neq X_1(\bb - \epsilon_1 + \epsilon_2)$ by induction, one has $X_1(\aa) \neq X_1(\bb)$, as desired.

\item $\mathbf{t \neq m, (\implies):}$ Assume $\aa$ and $\bb$ are adjacent. Observe that if $t\neq m$, then $m\in\Supp(\bb)$. Consider the element $\ww = \aa - \epsilon_m + \epsilon_s = \bb - \epsilon_m + \epsilon_t$. If $\ww$ is adjacent to either $\aa$ or $\bb$, then all three are connected by Conditoin \ref{cond: complete}. Now $\aa$ and $\ww$ fall into the case where $t=m$, so $X_1(\aa) = X_1(\ww)$ and $X_1(\ww) = X_1(\bb)$ by induction, so $X_1(\aa) = X_1(\bb)$.

Now assume that $\ww$ is adjacent to neither $\aa$ nor $\bb$. By Condition \ref{cond: 1parent1child}, $\bb + \epsilon_1 - \epsilon_m$ must be adjacent to $\aa + \epsilon_1 - \epsilon_m$. Moreover, all of $\aa, \bb$, and $\ww$ cover the element $\ff = \ww - \epsilon_1 + \epsilon_m = \bb-\epsilon_1 + \epsilon_t = \aa - \epsilon_1 + \epsilon_s$. By isotonicity of $X_1$, one has that $X_1(\ww) \cap X_1(\bb) = X_1(\ff)$ and $X_1(\ww) \cap X_1(\aa) = X_1(\ff)$, so $X_1(\aa) = X_1(\bb)$ as desired.

\item $\mathbf{t \neq m, (\impliedby):}$ Assume $\aa$ is not adjacent to $\bb$. Again consider the element $\ww = \aa - \epsilon_m + \epsilon_s = \bb - \epsilon_m + \epsilon_t$. Notice that $\aa$, $\bb$, and $\ww$ all share a child $\ff = \ww - \epsilon_1 + \epsilon_m = \bb-\epsilon_1 + \epsilon_t = \aa - \epsilon_1 + \epsilon_s$, so by Condition \ref{cond: twoParents}, at least one pair among the three must be adjacent in $G$. If either $\aa$ or $\bb$ is adjacent to $\ww$, the other cannot be by condition \ref{cond: complete}. Combining the induction hypothesis and the argument for the case when $t=m$ above gives the desired result. 
\end{itemize}
\end{proof}


==> sections/questions.tex <==
\section{Further Questions}\label{sec: questions}

In \cite{lohne2013many}, Lohne shows that in the three variable case, every minimal cellular resolution of $(x,y,z)^d$ gives rise to a polarization of $(x,y,z)^d$; and conversely, every polarization of $(x,y,z)^d$ gives rise to a minimal cellular resolution of $(x,y,z)^d$. We have seen, however, that there exist CW-complexes supporting a minimal free resolution of $\m^d$ whose graph of linear syzygies cannot give rise to a polarization (see Example \ref{ex: noIsotoneMapsLcomplex}). It is possible that if one restricts to \emph{polyhedral} cell complexes, then there is a corresponding generalization of Lohne's result.

\begin{question} Does every polyhedral cellular resolution of $\m^d$ give rise to a polarization of $\m^d$ via its graph of linear syzygies? Conversely, given a graph of linear syzygies corresponding to a polarization of $\m^d$, does there exist a (polyhedral) cellular resolution of $\mm^d$ with that graph of linear syzygies?
\end{question}

In addition, one might hope for some kind of algorithm to generate all possible polarizations of $\m^d$ quickly and efficiently. We hope our criterion for checking polarizations using hook tableaux in Theorem \ref{thm: spanningTree} is more amenable for such computations than the original spanning tree condition in Theorem \ref{thm: polsSyzEdges}. However, one must know exactly how to check the criteria in Theorem \ref{thm: isotone} in terms of hook tableaux to be able to generate all polarizations using this method. This leads to the following natural question.

\begin{question} Can one reinterpret conditions (G1)-(G4) in Theorem \ref{thm: isotone} in terms of hook tableaux?
\end{question}
